A High-Performance Design, Implementation, Deployment, and Evaluation of The Slim Fly Network

Novel low-diameter network topologies such as Slim Fly (SF) offer significant cost and power advantages over the established Fat Tree, Clos, or Dragonfly. To spearhead the adoption of low-diameter networks, we design, implement, deploy, and evaluate the first real-world SF installation. We focus on deployment, management, and operational aspects of our test cluster with 200 servers and carefully analyze performance. We demonstrate techniques for simple cabling and cabling validation as well as a novel high-performance routing architecture for InfiniBand-based low-diameter topologies. Our real-world benchmarks show SF's strong performance for many modern workloads such as deep neural network training, graph analytics, or linear algebra kernels. SF outperforms non-blocking Fat Trees in scalability while offering comparable or better performance and lower cost for large network sizes. Our work can facilitate deploying SF while the associated (open-source) routing architecture is fully portable and applicable to accelerate any low-diameter interconnect.

==> ad.tex <==
\section{Artifact Description}
\subsection{Artifact Identification}
Novel low-diameter network topologies such as Slim Fly offer significant cost and power advantages over the established Fat Tree, Clos, or Dragonfly. To spearhead the adoption of low-diameter networks, we design, implement, deploy, and evaluate the first real-world Slim Fly installation. We focus on deployment, management, and operational aspects of our test cluster with 200 servers and carefully analyze performance. We demonstrate techniques for simple cabling and cabling validation as well as a novel high-performance routing architecture for InfiniBand-based low-diameter topologies. Our real-world benchmarks show Slim Fly's strong performance for many modern workloads such as distributed deep neural network training, graph analytics, or linear algebra kernels. Our work can facilitate deploying Slim Fly while the associated (open-source) routing architecture is fully portable and can be used to accelerate any low-diameter interconnect.

Aside from the source code for our routing architecture integrated into the OpenSM InfiniBand subnet manager, the computational artifacts that support the reproducibility of our experiments include the custom alltoall implementation and deep neural neural network proxy workloads that we added to the t2hx benchmark suite. While reproducing the exact results of our real-world benchmarks will be impossible without access to the same Slim Fly installation, given that it is the first of its kind, the computational artifacts we provide enable the same evaluations to be performed on other deployments. Lastly, we include the scripts that facilitated the cluster deployment, run all benchmarks for the different routing configurations, and automated result extraction and plot creation.
\subsection{Reproducibility of Experiments}
Our work focuses on the design, implementation, deployment, and evaluation of the first real-world Slim fly installation, with the goal of spearheading the adoption of low-diameter networks. Firstly, In addition to the details in Section 3, we provide detailed information on the workflow of deploying our test cluster, which can be applied to any system based on the Slim Fly topology. Secondly, we describe the experimental workflow to obtain the exact results from our evaluation in Section 7, using the provided artifacts, if run on an equivalent system.

\subsection*{Experimental Workflow}
The cluster, which is hosted by the Swiss National Supercomputing Centre (CSCS), consists of 50 36-port, 56Gb/s IB SX6036 switches and 200 compute endpoints. To deploy it, the workflow involves several steps. Firstly, the topology outline is automatically generated through a script that is part of the computational artifacts. After placing all the switches and compute endpoints in the racks according to the outline, the 3-step process is used to wire everything up. To facilitate this, diagrams that show all intra-subgroup (step 1), inter-subgroup + intra-rack (step 2), and inter-rack cables (step 3) are generated. Then, the switch GUIDs are added to the topology outline, and the automatic verification script, which is also part of the computational artifacts, is used to verify that all cables are correctly wired up. We want to emphasise that this script could even be used on a live cluster, while going through the 3-step process, to immediately identify and flag any errors.

In order to evaluate the system and the new multipath routing algorithm, we deployed the subnet manager OpenSM v3.3.23 that updates all switch forwarding tables in accordance with the configured routing. The new algorithm, which is described in section 4.3, 5.1 and 5.2, is fully implemented in OpenSM under the alias lnmp and available under \url{https://github.com/nblach/opensm}. All benchmarks are evaluated for our new multipath routing algorithm, as well as DFSSSP, the defect standard multipath routing algorithm in IB, that leverages minimal paths only. 

For the benchmarks themselves we almost completely rely on the TSUBAME2 HyperX (t2hx) benchmark suite that is available under \url{https://gitlab.com/domke/t2hx}. We follow the installation guide outlined in the repository and update the configuration files and run scripts for our setting. We provide the updated configuration files and run scripts, which reflect the configurations outlined in Table 1, in the artifact (for convenience). We slightly modify the Graph 500 Benchmark by fixing the seed for the graph generation and reuse the same source vertex across all BFS runs. Additionally, we extend the Microbenchmarks with a custom implementation of MPI\_Alltoall and introduce a new collection of benchmarks, the DNN Proxies, to the suite. These additional benchmarks are installed, configured and executed in the exact same fashion as the other ones of the t2hx benchmark suite. Note that the three deep neural network proxy applications (Performance displayed in Figure 13) are a subset of the proxy applications available under \url{https://github.com/spcl/DNN-cpp-proxies}, with setup instructions provided under this link.

After the necessary installation and configuration steps have been performed, the remaining workflow, which comprises routing instantiation, benchmark execution, data cleaning, and result visualization, is fully automized by the provided scripts. The scripts instantiate each routing algorithm once with 1, 2, 4, and 8 layers, respectively, and run each combination of benchmark and routing configuration 5 times, with Microbenchmarks for at least 100 iterations. The output of the benchmarks is collected in a central directory, from which the plotting script can then extract the relevant information that should be displayed. 

\subsection*{Estimation of Execution Time}
We run each benchmark 5 times for each of the 8 routing configurations, so each benchmark is executed a total of 40 times, except the Microbenchmarks that are only run once per routing configuration, as they already run for at least 100 iterations. The execution time of each run for each benchmark is limited to 15 minutes. However, as can be seen in Figure 13, most take significantly less time to execute. We estimate the overall execution time to be around $3.5$ days.

\subsection*{Expected Results and Relationship to the Results in the Submission}

Reproducing the exact results is possible by either constructing a cluster based on our installation, or by accessing the same Slim Fly cluster. Otherwise, results with the same performance trends can be obtained for other deployments, if the experiments are run for the same configurations as listed in Table 1. Table 1 further shows the expected results, specifically it shows the metric and scaling behaviour that is evaluated for each benchmark configuration. In the submission, only the best-performing routing configuration (for each benchmark/baseline) is plotted. The artifacts contain the commands to the plotting script that will display the expected results in the same format as in the submission. If coupled with our complete result logs (also included), they will produce identical results.


